Advanced Model Consistency Restoration with Higher-Order Short-Cut Rules

Sequential model synchronisation is the task of propagating changes from one model to another correlated one to restore consistency. It is challenging to perform this propagation in a least-changing way that avoids unnecessary deletions (which might cause information loss). From a theoretical point of view, so-called short-cut (SC) rules have been developed that enable provably correct propagation of changes while avoiding information loss. However, to be able to react to every possible change, an infinite set of such rules might be necessary. Practically, only small sets of pre-computed basic SC rules have been used, severely restricting the kind of changes that can be propagated without loss of information. In this work, we close that gap by developing an approach to compute more complex required SC rules on-the-fly during synchronisation. These higher-order SC rules allow us to cope with more complex scenarios when multiple changes must be handled in one step. We implemented our approach in the model transformation tool eMoflon. An evaluation shows that the overhead of computing higher-order SC rules on-the-fly is tolerable and at times even improves the overall performance. Above that, completely new scenarios can be dealt with without the loss of information.

==> imports.tex <==
\usepackage{graphicx}
\usepackage{listings}
\usepackage{enumitem}
\usepackage{import}
\usepackage{acronym}
%\usepackage{todonotes}[outline]
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage[style=british]{csquotes}
%\usepackage{hyperref}
%%%%%% To display ORCID Logo with link, Please add below definition and copy the ORCID_Color.eps in the manuscript package %%%%%
\makeatletter
\RequirePackage[bookmarks,unicode,colorlinks=true]{hyperref}%
   \def\@citecolor{blue}%
   \def\@urlcolor{blue}%
   \def\@linkcolor{blue}%
\def\UrlFont{\rmfamily}
\def\orcidID#1{\smash{\href{http://orcid.org/#1}{\protect\raisebox{-1.25pt}{\protect\includegraphics{figures/orcid_color.eps}}}}}
\makeatother

% If you use the hyperref package, please uncomment the following two lines
% to display URLs in blue roman font according to Springer's eBook style:
\usepackage{xcolor}
%\renewcommand\UrlFont{\color{blue}\rmfamily}   % I disabled the blue links. If you do not agree with this, let us know
\usepackage[noabbrev, capitalise]{cleveref}
\usepackage[noend]{algpseudocode}
\usepackage[Algorithm]{algorithm} 
\usepackage[most]{tcolorbox} % colored box for research challenges
\usepackage{float}
\usepackage{adjustbox}
\usepackage{cite}
\usepackage{tikz}
